Probing gravity with a joint analysis of galaxy and CMB lensing and SDSS spectroscopy

We present measurements of $E_G$, a probe of gravity from large-scale structure, using BOSS LOWZ and CMASS spectroscopic samples, with lensing measurements from SDSS (galaxy lensing) and Planck (CMB lensing). Using SDSS lensing and the BOSS LOWZ sample, we measure $\langle{E_G}\rangle=0.40^{+0.05}_{-0.04}$ (stat), $\pm 0.026$ (systematic), consistent with the predicted value from the Planck $\Lambda$CDM model, $E_G=0.46$. Using CMB lensing, we measure $\langle{E_G}\rangle=0.46^{+0.08}_{-0.09}$ (stat) for LOWZ (statistically consistent with galaxy lensing and Planck predictions) and $\langle{E_G}\rangle=0.39^{+0.05}_{-0.05}$ (stat) for the CMASS sample, consistent with the Planck prediction of $E_G=0.40$ given the higher redshift of the sample. We also study the redshift evolution of $E_G$ by splitting the LOWZ sample into two samples based on redshift, with results being consistent with model predictions. We estimate systematic uncertainties on the above $\langle{E_G}\rangle$ numbers to be $\sim 6$% (when using galaxy-galaxy lensing) or $\sim 3$% (when using CMB lensing), subdominant to the quoted statistical errors. These systematic error budgets are dominated by observational systematics in galaxy-galaxy lensing and by theoretical modeling uncertainties, respectively. We do not estimate observational systematics in galaxy-CMB lensing cross correlations.

==> referee_response <==
Assistant Editor's Comments:
Editor
Comments to the Author:
> Our similarity checker shows that Section 3.1 is similar to another
> paper. Could you please reword it.

Scientific Editor's Comments:
Editor
Comments to the Author:
> Our automated plagiarism check showed that some material is very
> similar to other papers. e.g. Section 3.1 is identical to a paragraph
> in your paper Monthly Notices of the Royal Astronomical Society,
> Volume 464, Issue 2, p.2120-2138 (arXiv:1606.08841). Section 3.3 also
> duplicates material from this paper. Please endeavour to avoid direct
> quotation of material from other papers. From the MNRAS Instructions
> to Authors, Section 2.6: "Any re-use of material which has previously
> been published 

- We apologize for the repeated content. This is standard material associated with use of the SDSS
- collaboration data here and in the paper you mentioned (arXiv:1606.08841). We have edited the 
- material in section 3.1 and 3.3 to reduce textual overlap while retaining the required citations.

Reviewer's Comments:
Reviewer: 1

Comments to the Author
> The authors present a measurement using the Eg estimator - a
> combination of lensing, galaxy clustering and RSD data - to test for
> consistency between observations and LCDM. They find marginal
> agreement between the two at ~2.5sigma with optical weak lensing data,
> and a smaller difference (partially due to larger uncertainties) when
> CMB lensing data is used instead. 

> The analysis is presented clearly, and the methodology is sound. 

> The paper is worthy of publication in MNRAS with minor revision.

- We thank the referee for a very positive report, that has helped in
- improving the quality of the paper. 

- We respond to the Referee's comments below. Changes in the paper are
- highlighted in green color.

Major Comments:

> 1) Covariance treatment: 
> a) While I understood the idea of using the distribution of the
> measured values from jackknives to estimate the error on the Eg, I
> didn't see how the covariance that was used in each jackknife was
> estimated. (eg L43 'we do so for each jackknife region separately
> using the diagonal of the covariance') Similarly how was the L60 full
> covariance for RSD calculated?

- We always use the jackknife covariance for the measurements. We have made 
- minor edits in section 2.7 to highlight this.
- We first get the covariance using all jackknife regions and then use that covariance
- even when fitting an individual jackknife region. While the covariance for 
- a jackknife region is slightly larger (by ~1%) than the full sample, it 
- does not change the best fit values of parameters that we use.

> b) The extra variance due to a noisy estimate of the covariance is
> normally very amenable to checking with simple toy model
> simulations. Have the authors done such a test to confirm that by
> using the diagonal terms of the covariance in the jackknife split, it
> is right to have no correction? The existing argument is unsatisfying
> in that it sounds like "we don't know the answer, so we go with the
> smaller error bars"

- We have added a statement to justify the omission of Hartlap factor.
- We have also checked with simulations that the Hartlap correction
- is of order 1.5% when using diagonal errors.

> 2) Treatment of sys errors in the abstract: 
> - It's unclear whether the 5% of the last sentence is included in the
> earlier quoted numbers or not. 
- Systematic errors were included in the statement. Please note that
- that statement has been removed (see response to comment below)

> -It is inappropriate to the deviation with statistical errors only,
> rather than the significance of the deviation given both stat and sys
> errors. 
- We have removed the statement, especially since we made changes in the
- RSD analysis (described later in this response), as a result of which
- the mean value and noise in EG increased, reducing the discrepancy with
- the Planck predictions. 

> Why do some Eg numbers quote the sys budget, and some do not?
- We agree with the referee that we were not consistent in quoting the
- systematic errors in the previous version. In the current version we only quote the
- statistical errors, while providing a complete description of the systematic error budget,
- including the dominant terms and how they compare with the statistical errors. 
- The systematic errors we identified are smaller
- than the statistical errors and do not significantly change the total
- error budget. To be clear, our results suggest ~2% systematic error
- due to modeling uncertainties that affect the results using both CMB
- and galaxy-galaxy lensing. In the galaxy-galaxy lensing, there is an additional ~5%
- uncertainty due to photometric redshifts and shear calibration,
- though photometric redshifts dominate this budget. 
- In this work, we do not estimate the systematic uncertainties in galaxy-CMB lensing
- cross correlations. 

> 3) Systematic errors: Why doesn't Table 1 include the systematic
> errors?
 > It'd also be useful to tabulate/clarify the total systematic error in
 > the different Eg measurements, and where it's sourced from. A 2%
 > number is quoted in 3.2, in 4.2 from a different source of
 > systematics, and 5% from sdss lensing redshift. Other times the
 > systematics are quoted as ~2%. It's not clear where the ~2% comes
 > from; two 2% terms would seem to be more like 3%. Clarifying the
 > systematics budget would be valuable. 
- We have added a line in the caption of table 1 clarifying the
- systematic budget. Systematics levels for different samples are very
- similar, hence we do not think quoting separate values for each are necessary.

> 4) Sec 3.4: How much would the uncertainties increase if l<400 was
> cut? It would be worth commenting on this in the text. 

- The EG measurement using scales corresponding roughly to l<400 is quoted when
- comparing with the Pullen+2016 results. We have also added this 
- value in Table 1. Errors change from ~12.5% to ~16% while the central
- values shift by <0.5\sigma.

> 5) p11: "we checked that it does not affect our results as the
> off-diagonal elements of the covariance matrix are sub-dominant"  How
> was this checked? I didn't see a description of this check in the
> covariance section. 

- We checked this by recomputing the EG with the full covariance. We have
- added a line in the text clarifying this.

> Minor Comments: 

> 1) "randoms" in L35 seems to be jargon.

- We have added a description after equation 8.

> 2) Sec 2.6: While the total correction is shown in a later figure,
> it'd be interesting to comment on the relative size of the different
> terms here (or later).

- We have added a desciption in section 4.3 (page 10), when discussing
- fig. 5


> 3) 4.1: I found the comparison with previous work a little jumbled,
> although it can be left as is.
- We have opted to leave the discussion as is. 

Other changes unrelated to referee comments:
- Text in section 3.1 and 3.3 describing SDSS and BOSS data has been
- slightly edited to avoid overlap with similar text in our earlier papers.

- We have also changed the scales for fitting the RSD measurements to
- get the growth rate $f$. In the previous version of the paper, we were using a minimum
- scale of 28 Mpc/h in the fits, while in the current version it is set
- to 35 Mpc/h to avoid scales where the model does not work perfectly. This
- leads to a decrease in the values of $f$ of order 0.5-1 sigma for
- the LOWZ sample and its subsamples, which in turn increases EG.
- In addition we have also added the systematic uncertainty in the RSD
- analysis to our systematics error budget. 

